FIVB ranking: Misstep in the right direction

This work presents and evaluates the ranking algorithm that has been used by Federation Internationale de Volleyball (FIVB) since 2020. The prominent feature of the FIVB ranking is the use of the probabilistic model, which explicitly calculates the probabilities of the future matches results using the estimated teams' strengths. Such explicit modeling is new in the context of official sport rankings, especially for multi-level outcomes, and we study the optimality of its parameters using both analytical and numerical methods. We conclude that from the modeling perspective, the current thresholds fit well the data but adding the home-field advantage (HFA) would be beneficial. Regarding the algorithm itself, we explain the rationale behind the approximations currently used and show a simple method to find new parameters (numerical score) which improve the performance. We also show that the weighting of the match results is counterproductive.

==> Common.Files/tikz.definitions.tex <==
% Define a few styles and constants

% Function block
\tikzstyle{rect_my} = [draw, rectangle, minimum width=2cm, text width=1.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{square_my} = [draw, rectangle, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{square_my_graph} = [draw, rectangle, minimum width=1.2cm, text width=1cm, fill=gray!15, 
  text centered,  minimum height=1.2cm]
\tikzstyle{circle_my} = [draw, circle, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{circle_my_graph} = [draw, circle, minimum width=1.1cm, text width=.8cm, fill=gray!15, 
  text centered]
\tikzstyle{cloud_my} = [draw, shape=cloud, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=1cm]

% Point
\tikzstyle{point_my} = [draw=none, minimum width=0cm, text width=0cm, fill=none, 
  text centered,  minimum height=0cm]    
\tikzstyle{line_my} = [draw, -latex]    
% Boxes
\tikzstyle{box_my}=[draw, minimum size=2em, text width=4.5em, text centered]
\tikzstyle{bigbox_my}=[draw, inner sep=15pt]
\tikzstyle{arrow_my} = [thick,->,>=stealth]
\tikzstyle{noarrow_my} = [thick,-,=>stealth]

%%%
\newcommand{\jumpline}[2]{
\path(#1.east) --(#2.west)  coordinate[pos=0.4](mid);
\draw[-latex] (#1.east) -| (mid) |- (#2.west);
}

==> figures/Fig.Integration.tex <==
\begin{tikzpicture}

% Axis
\draw[->] (-1.5,0) -- (1.7,0) node[below] {$z$};
\draw[->] (0,-0.5) -- (0,1.5) node[left] {$u$};

% Line  y = a * x = b
% a = 0.5; b = 1 
\draw[blue, thick] (-1.5,0.25) -- ++(2.5,1.25) node[right,black] {$u=c+z\sqrt{2v}$};

% Shaded area below the line
\fill[blue, opacity=0.3] (-1.5, -1.5) -- (-1.5, 1) plot[domain=-1.5:1.5, samples=100] (\x, {0.5*\x + 1}) -- (1.5, 1) -- (1.5, -0.5) -- (-1.5,-0.5) -- cycle;


% Tick at (0,1)
\draw[red, thick] (0,1) -- ++(0.1,0) node[right,black] {$c$};
% Tick at (-1,0)
% \draw[red, thick] (-1,0) -- ++(0,0.1) node[right,black] {$C2$};

% draw line from (0,0) to (-ab(a^2+1), b/(a^2+1) )  
\draw[blue] (0,0) -- (-0.4, 0.8);

\node[left, rotate=0] at (-0.2,0.4) {$d$};



\end{tikzpicture}
